Extending 3-DoF Metrics to Model User Behaviour Similarity in 6-DoF Immersive Applications

Immersive reality technologies, such as Virtual and Augmented Reality, have ushered a new era of user-centric systems, in which every aspect of the coding--delivery--rendering chain is tailored to the interaction of the users. Understanding the actual interactivity and behaviour of the users is still an open challenge and a key step to enabling such a user-centric system. Our main goal is to extend the applicability of existing behavioural methodologies for studying user navigation in the case of 6 Degree-of-Freedom (DoF). Specifically, we first compare the navigation in 6-DoF with its 3-DoF counterpart highlighting the main differences and novelties. Then, we define new metrics aimed at better modelling behavioural similarities between users in a 6-DoF system. We validate and test our solutions on real navigation paths of users interacting with dynamic volumetric media in 6-DoF Virtual Reality conditions. Our results show that metrics that consider both user position and viewing direction better perform in detecting user similarity while navigating in a 6-DoF system. Having easy-to-use but robust metrics that underpin multiple tools and answer the question ``how do we detect if two users look at the same content?" open the gate to new solutions for a user-centric system.

==> _Sec_3_challenges.tex <==
\begin{figure*}[h!]
	\centering
    \hspace{-2em}
	\subfigure[Mean Ratio Overlap.]{
	\includegraphics[width=0.5\textwidth]{Figure_Jrn/PC_Longdress_Over_time_overlap_set_1.png}}
	\quad
    \hspace{-2em}
	\subfigure[Mean Relevant Users.]{
		\includegraphics[width=0.5\textwidth]{Figure_Jrn/PC_Longdress_Over_time_users_set_1.png}}
		\\
    \hspace{-2em}
	\subfigure[Precision.]{
		\includegraphics[width=0.5\textwidth]{Figure_Jrn/PC_Longdress_Over_time_precision_set_1.png}}
		\quad
    \hspace{-2em}
	\subfigure[GDI.]{
		\includegraphics[width=0.5\textwidth]{Figure_Jrn/PC_Longdress_Over_time_gdi_set_1.png}}
	\caption{Spherical clustering over time (chunk = 1 sec.) results per sequence PC1 (\textit{Longdress}). Comparison between Ground-truth, and single feature metric ($w_1$, $w_2$, $w_3$ and $w_4$). }
	\label{Fig_overTime_set1}
	\vspace{-1.5em}
\end{figure*}

\section{Challenges}
\label{sec_challenges}
\lt{given the flow of the paper I am thinking that we could have B C and A as order of the section. I feel that you would talk immediately about the 6dof and users behaviour. Then you say that this similarity can be used in tools to extract objective measurements of the users' similarity and in this paper we will be using it in the clustering. }
In this work, we investigate behavioural similarities among users via a clique-based clustering proposed in the \cite{rossi2019spherical}. This algorithm has been proposed to identify users who are attending the same portion of an omnidirectional content in a 3-\ac{DOF} system. We are aiming at extending the applicability of this tool to \sdof users. However, due to the new setting and locomotion functionalities, there are some new challenges that need to be addressed. \noteSR{not sure if having also the following part here:} In the following, we first define our assumption of similarity among users while navigating in a \sdof environment. Then, we propose \noteSR{?} a ground-truth user similarity metric highlighting its limitations, and therefore the need to find a simpler and reliable proxy for it. Finally, we show the need of similarity metric for behavioural analysis via a  clique-based clustering approach. \lt{havent checked as I would first check if we keep this order or not. }
\subsection{Behavioural analysis via clique-based clustering (?) \lt{Clustering as tool for behavioural analysis}}
\lt{I would spend few lines jsut to mention that we need to assess users' similarity in an objective way and clustering can be one. Then say that as shown in XX to ensure meaningful graph clique-based clustering was proposed. }
The clique-based clustering is a graph algorithm that identifies optimal sub-graphs of inter-connected nodes. The first step in order to use this tool is   to construct a reliable graph that models the user behaviour \lt{maybe we can say what this means: graph showing interconnections between users that dispaly the same content? you say it later but more technically so the key concept might slip away. }. Given a set of users who are experiencing the same content, we can represent their movements in a time-window $T$ as a set of graphs $\{ \mathcal{G}_t\}_{t=1}^T$. Each unweighted and undirected  graph $\mathcal{G}_t = \{\mathcal{V}, \mathcal{E}_t, \text{A}_t \}$ represents behavioural similarities among users at time $t$, where $\mathcal{V}$ and $\mathcal{E}_t$ denote the node and edge sets of $\mathcal{G}_t$, respectively. Each node in  $\mathcal{V}$ corresponds to a user interacting with the content. Each edge in $\mathcal{E}_t$ connects neighbouring nodes defined by the binary adjacency matrix $\text{A}_t$. A key aspect to consider is how to define the neighbourhood of each user. Assuming that users are neighbours if they are displaying similar content, we can formally define the adjacency matrix $\text{A}_t$ as follow:
\begin{equation}
	\text{A}_t(i,j) = 	 
	\begin{cases} 
	1,    & \mbox{if } w_t(i,j) \leq G_{th} \\ 
	0, & \text{otherwise}. \\
	\end{cases} 
\end{equation}
where $w_t(i,j)$ is a similarity metric between user $i$ and $j$ and $G_{th}$ is a thresholding value. On this final graph, the clique-based clustering algorithm can be applied to identify a set of users all connected (\ie clique), and therefore with similar behaviour. \\

Identifying a generic and reliable metric $w(i,j)$ that approximates behavioural similarities among users who experience a \sdof content is a key step to enable a user behavioural analysis.

\noteSR{maybe would be better to find a way to discard $t$} 
\lt{I don;t mind too much having the $t$ but one option could be to present the graph and all the definition for one graph only and one single pointcloud frame, then you say that this can be extended over time, leading to  set of graphs $\{ \mathcal{G}_t\}_{t=1}^T$. Depending on the space we have, it could also be nice to have a figure that show the point cloud, the users and the graph associated to it or something that gives an immediate undertansing. This is however very optional at the moment. }

\subsection{User Similarity in 6-DoF}
We assume that users are similar if they are attending a similar portion of the content: this corresponds to a consistent overlap between their viewport. In a \tdof system, the distance between the projection of viewport centre on the content (\ie viewing sphere) can be used as a proxy of viewport overlap among users \cite{rossi2019spherical}. %\lt{here you talk about overlap but we introduce the ground-truth later in the next section. Maybe we could have the next section first and then this one? Or if here you only want to talk about the user behaviour and trajectory I would remove this first part. }
In particular, the geodesic distance has been proved as a reliable similarity metric $w(i,j)$ such that low value indicates high similarity between \tdof users. This is not true in a \sdof system: the more degrees of freedom is given to the user, the more challenging becomes the system. %Thus, the viewport centre alone is not sufficient to characterise the user behaviour. %Therefore, we are aiming at defining a simple and straightforward solution that takes into account the new settings and locomotion functionalities of a 6-\ac{DOF} scenario but that approximates viewport overlap.
%Meaning also that the distance between viewport centres of different users alone might not be sufficient to identify similarity among viewers.
 %In a \sdof setting, the distance between the user and immersive content can change over time due to the added degrees of freedom. As in the \tdof setting, a small distance between two viewport centres might  suggest  a  high  overlap between the corresponding user viewports, and therefore a high similarity. However this  might not necessarily be  true  if  they  are  at  a  very  different  relative  distance  from the volumetric content. 
 %To better understand this concept, 
 \begin{figure}[t!]
	\centering
    \includegraphics[width=0.4\textwidth]{Figure_Jrn/6DoF_system.png} 
	\caption{An example of \sdof~trajectories projected in a 2D domain for user $i$ and $j$. In the circle, a snapshot at time $t$ where coloured triangles represent viewing frustum per user. }
	\label{fig_6dofnavigation}
\end{figure}
 Figure~\ref{fig_6dofnavigation} shows an example of two users navigating in a \sdof system. In the bottom part of the figure, there are navigation trajectories of two users $i$ and $j$ projected on a 2-D domain (\ie floor). Each point $x_t$ represents the spatial coordinates (\ie [x,y,z]) on the floor while each associated vector symbolises the viewing direction.  In the top part of Figure~\ref{fig_6dofnavigation}, we have instead a snapshot of a specific time instant $t$. In more details, triangles represent the \emph{viewing frustum} per user which indicate the area within the user viewport, and $r_t$ is the distance between the user and the volumetric content. We have also depicted the viewport centre $p_t$ projected on the displayed volumetric object. Given the two users $i$ and $j$ at time $t$, with $r^i_t \gg r^j_t$, the latter, who is very close to the object, is visualising a very focused and detailed part of it; conversely, user $i$ is pointing to the same area but from further distance, thus she/he is experiencing the content differently. The small distance $D_t(i,j)$ between viewport centres $p_t^i$ and $p_t^j$ might suggest a high similarity (\ie high viewport overlap) between the corresponding users, which might not be true in this case, due to the two different prospective and distance of users. Thus, the viewport centre alone is not sufficient to characterise the user behaviour, but distance $r$ and the spatial coordinates on the virtual floor $x$ are also needed. Given the above notation, we can formally define the navigation trajectory for a generic \sdof user $i$ as $ \{(x^i_1,p^i_1,r^i_1), (x^i_2,p^i_2,r^i_2), \dots,(x^i_n,p^i_n,r^i_n)\}$ \noteSR{maybe should I move this sentence above?}. This information is also crucial to define a simple and straightforward similarity metric among users in this new setting.% approximates viewport overlap to be used as similarity metric
%, we need to take into account not only the position of the viewport centre $p$ (as it was in a 3-\ac{DOF}) but also the other relevant information: user position on the floor $x$ and relative distance $r$ to the volumetric content.
\lt{we may want to discuss on this section before editing but you can either show first the 3dof trajectory, comment on the fact that the distance from teh viewport center is quite indicative of the users behavior and then comment on 6dof --highlighting the extra variables and degree of freedom and the problems that follow. Or you can talk directly about the 6dof and the trajectory since the beginning and highglight the problem in measuring the similarity.}


\subsection{Overlap Ratio as the ground-truth metric}
\label{sec_overlapRatio}
Since we are interested in capturing viewers that are attending similar volumetric content at the same time instance, the straightforward measure that could show this behaviour is the overlap among viewports. Given two users $i$ and $j$ described above in Figure~\ref{fig_6dofnavigation}~(top part), we can define their displayed viewport as $\mathcal{S}_t^i$ and $\mathcal{S}_t^j$, the set of points of the volumetric content falling within the viewing frustum cast by user $i$ and $j$. Then, we denote the overlap set by  $\mathcal{S}_t^{i} \cap \mathcal{S}_t^{j}$, defined as the portion of points displayed by both users. Equipped with the above notation, we can now introduce a key metric for the analysis: the \textit{overlap ratio} $O(i,j)$. The latter is defined as the cardinality of the overlap set, normalised by the cardinality of the set containing all points of the volumetric content visualised by both users. More formally, the overlap ratio in a specific time $t$ is:
\begin{equation}
    O_t(i,j) = \frac{|\mathcal{S}_t^{i} \cap \mathcal{S}_t^{j}|}{|\mathcal{S}_t^{i} \cup \mathcal{S}_t^{i} |}
\end{equation}
where $\mathcal{S}_t^i$ and $\mathcal{S}_t^j$ are the displayed viewport of users $i$ and $j$, respectively. The higher is the overlap ratio, the higher is the similarity between users, and vice versa. Even if this metric is a clear indicator of how much similar users are with respect to their displayed content, its evaluation is not trivial, and intensely time-consuming. For instance, the overlap ratio between two users requires 0.8986 seconds per frame on average on a \noteIV{which machine? laptop? pc?} \noteSR{I did on UCL server so maybe I would say machine to be generic?}; the operation needs to be computed for all the possible combinations of users, leading to large overhead which does not meet requirements for real-time and scalable applications. A new measure is thus needed to perform clustering in near real-time. \noteSR{0.8986 sec average computational time to evaluate overlap ratio btw two users in a single frame - it has to be multiple for the number of all the possible couples $C_{n}^2$.}  \noteSR{@Irene, please feel free to change and add more details.} In the following, we will use this metric as the ground truth of overlap among users, and we investigate the use of different weights as a proxy for viewport overlap.
% However, finding a simpler and more straightforward solution as a proxy for viewport overlap would be beneficial for enabling real-time and scalable applications. 
\lt{this is very well self-contained so we could have it before the "user similarity in 6dof", where we than say that the overcome the computational burden we could have an approximation. In the case of 3dof the cneter distance was the proxy but in 6dof this would not be a good reflection of the ground truth etc. Yo can then conclude that these similarities metrics can be used in many wauys to study users beahvior and in your case you apply it to the clustering. What I like in having the clustering at the end is that it emphasize the concept that the clustering is not the core of the work and your metrics could work in general and not onluy for the clsutering. }







==> _Sec_3_old.tex <==
\section{Background notions}
\label{sec:II_background}
In this work, we investigate similarities among users via a clique-based clustering proposed in \cite{rossi2019spherical}. This algorithm has been proposed to identify users who are  attending the same portion of an omnidirectional content in a 3-\ac{DOF} system. We are aiming at extending this tool also for analysing users in a \sdof system. As argued in \cite{rossi2021anewchallenge}, due to the new settings and locomotion functionalities of 6-\ac{DOF}, a new metric that  reliably reflects users similarities during the navigation is needed. In this section, we first define \sdof navigation trajectory highliting the main difference with a \tdof scenario. Then, we describe the clustering algorithm for behavioural analysis in \tdof showing the intrinsic need of finding a proper similarity metric for \sdof user.


\subsection{Navigation Trajectory in a 6-DoF Environment}
\label{sec_6DOFsystem}
The user behaviour can be identified by the  spatio-temporal sequences of their movements within the virtual environment, namely \emph{navigation trajectories}. \noteSR{I took this part from ICIP paper}
In a \tdof~scenario, the trajectory of a generic user $i$ can be formally denoted by the sequence of the user's viewing direction over time $ \{p^i_1,p^i_2,..,p^i_n\}$ where $p^i_t$ is the center of the viewport projected on the immersive content (\ie spherical video) at timestamp $t$. 
The point $p$ can be represented in spherical coordinates by $[\theta, \phi, r]$ where $\theta \in  [0,2\pi]$ is the azimuth angle (or longitude), $\phi \in [0, \pi]$  the polar angle (or latitude), and $r$ is the distance between the point (viewport center projected on the immersive content) and the origin (user position). In a \tdof~scenario, users are positioned at the centre of the spherical content; thus, $r$  is constant during the interaction.  As a consequence, the viewport centre alone is highly informative of the user behaviour, and can be used as a proxy of viewport overlap among users~\cite{rossi2019spherical}. In particular, if the distance between viewport centres is low, the similarity between users corresponds to high viewport overlap. \noteSR{I didn't have this before because we thought it might be confusing the notation}

In a \sdof setting, however, the distance between the user and immersive content can change over time due to the added degrees of freedom. Thus, the more degrees of freedom are given to the user, the more challenging becomes the system, and the description of user navigation within it. The viewport centre alone is not more sufficient to characterise the user behaviour in a \sdof scenario. Meaning also that the distance between viewport centres of different users alone might not be sufficient to identify similarity among viewers. In a \sdof setting, indeed, the distance between the user and immersive content can change over time due to the added degrees of freedom. As in the \tdof setting, a small distance between two viewport centres might  suggest  a  high  overlap between the corresponding user viewports, and therefore a high similarity. However this  might not necessarily be  true  if  they  are  at  a  very  different  relative  distance  from the volumetric content. To better understand this concept, we show in Fig.~\ref{fig_6dofnavigation} an example of two users navigating in a \sdof system.
\begin{figure}[t]
	\centering
    \includegraphics[width=0.5\textwidth]{Figure_Jrn/6DoF_system.png} 
	\caption{An example of \sdof~trajectories projected in a 2D domain for user $i$ and $j$. In the circle, a snapshot at time $t$ where coloured triangles represent viewing frustum per user. }
	\label{fig_6dofnavigation}
\end{figure}
In the bottom part of the figure, there are shown the navigation trajectories of two users $i$ and $j$ projected on a 2-D domain (\ie floor). Each point $x_t$ represents the spatial coordinates (\ie [x,y,z]) on the floor while each associated vector symbolise the viewing direction. In the top part of Fig.~\ref{fig_6dofnavigation}, we have instead a snapshot of a specific time instant $t$. In details, the user's \emph{viewing frustum} is represented by triangles, which indicate the area within the user's viewport and $r^i_t$ is the distance between user and the volumetric content. We have also depicted the viewport center $p^i_t$ projected on the displayed volumetric object. Given the users $i$ and $j$ at time $t$  with $r^i_t \gg r^j_t$, the latter, who is very close to the object, will visualise a very focused and detailed part of it; conversely, user $i$ is pointing to the same area but from further distance, thus she/he will experience the content differently. The small distance $D_t(i,j)$ between viewport centres $p_t^i$ and $p_t^j$ might suggest a high similarity between the corresponding users, which is not true in this case since they are displaying the volumetric content from two very different positions and at a very different distance. Therefore, the distance $r$ between the viewer and the object is now crucial to identify the actual displayed portion of the content. 
In fact, \sdof~navigation trajectories cannot be merely represented only by time and viewport's center position, as the point of origin (\ie user position) is also needed. Therefore,  we define the navigation trajectory for a generic \sdof~user $i$ as $ \{(x^i_1,p^i_1,r^i_1), (x^i_2,p^i_2,r^i_2), \dots,(x^i_n,p^i_n,r^i_n)\}$. At a generic time $t$ in addition to the viewport center $p^i_t$ projected on the displayed volumetric object, there are also $x^i_t$ which represents the spatial coordinates (\ie [x,y,z]) of the user in the \ac{VR} environment and the distance $r^i_t$ as the distance between user and viewport center $p^i_t$.


\subsection{Behavioural Analysis via user clustering}


Given the navigation trajectories for a set of \sdof users while experience the same volumetric content, we can model the general behaviour in a time-window $T$ as a set of graphs $\{ \mathcal{G}_t\}_{t=1}^T$, similarly to \cite{rossi2019spherical}. Each unweighted and undirected  graph $\mathcal{G}_t = \{\mathcal{V}, \mathcal{E}_t, \text{W}_t \}$ represents  the set of users navigating over time, where $\mathcal{V}$ and $\mathcal{E}_t$ denote the node and edge sets of $\mathcal{G}_t$, respectively. Each node in  $\mathcal{V}$ corresponds to a user interacting with the volumetric content at instant $t$. Each edge in $\mathcal{E}_t$ connects neighbouring nodes. A key aspect to consider is how to define the neighbourhood of each user. Therefore, a measure of similarity that assesses how much viewers behave similarly to each other is needed. The binary matrix $\text{W}_t$ define indeed which nodes are connected with $w_t(i,j)=1$ if the similarity metric between the corresponding users is above (or below based on the definition) at a given threshold. On the constructed graph, the clique-based clustering algorithm can be apply to identify cliques of users all connected and therefore, with a similar behaviour. The first step is to identify a reliable metric of similarity. 













==> _Sec_4_ProblemStatement.tex <==

\section{Problem statement}%: User Similarity in 6-DoF}
\label{sec:problem_statement}
%In this section, we define the challenge of finding a user similarity metric due to the new settings and locomotion functionalities of 6-\ac{DOF}. Then, we introduce 



==> _Sec_7_CaseStudy.tex <==
\section{Case study}
\label{Sec_caseStudy}
\begin{figure}[ht]
	\centering
	\hspace{-.5em}
	\subfigure[VV1]{
	\includegraphics[width=0.4\textwidth]{Figure_Jrn/PC_Nico_singleClusters.png}}
	\\
    \hspace{-2em}
	\subfigure[VV2]{
		\includegraphics[width=0.4\textwidth]{Figure_Jrn/PC_Fredrick_singleClusters.png}}
    \hspace{-2em}
	\caption{Single-user cluster per sequence VV1 (\textit{Nico}) and VV2 (\textit{Sir Fredrick}) obtained via spherical clustering based on overlap ratio, and a subset of proposed similarity metrics ($w_1$, $w_5$, $w_7$ and $w_8$).}
	\label{Fig_Vsense_2}
	\vspace{-1em}
\end{figure}
The above study has been carried out with a dataset only and we are therefore interested in understanding if insights from the above study could be applied to other human-like datasets. To show that our study generalises to datasets, we now investigate the proposed metrics on 
%To show the flexibility of our proposed similarity metrics, we now apply them to a different dataset. In particular, we select 
the dataset presented in \cite{zerman2021user}. Authors have collected navigation trajectories of 20 users while displaying volumetric content in an Augmented Reality (AR) scenario. Similarly to the previously analysed dataset presented in Section~\ref{sec_dataset}, a single object of interest was placed in the scene. Specifically, two dynamic volumetric human body sequences represented as 3D meshes with texture information were used: \textit{Nico} (VV1) and \textit{Sir Frederic} (VV2) in Figure~\ref{Fig_HumanBodyDataset2}, respectively. In order to conduct our study, both the sequences were kindly made available by Volograms upon request \cite{volograms2021,volgrams_website}. The navigation data have been collected in a remote scenario through an Android AR application, which allowed users to display the volumetric content from any desired location and portable device (e.g., smartphone). Participants were also free to display the volumetric content how they most preferred.  
Thus, the main differences with the previously analysed dataset are the following: the different format of volumetric content (3D mesh instead of point cloud), different immersive scenario (AR instead of VR application) and the heterogeneity of viewing devices (any smartphone device instead of a specific HMD). In particular, the 3D mesh content does not allow for a simple formulation of the overlap ratio as we have described it in Section~\ref{sec_overlapRatio}. For consistency, we convert the sequences from 3D meshes to point clouds by discarding edge information and only keeping vertices as points; we discuss the inherent challenges to define our ground-truth metric in Section~\ref{sec_discussion}.  %In particular, the new content format does not allow to evaluate the overlap between the displayed portion of two different users. In detail, to evaluate our ground-truth metric as described in Section~\ref{sec_overlapRatio}, we extract only the spatial information of the two volumetric videos and converted in point cloud \noteSR{to discuss with @Irene}. 

\begin{figure}[!t]
    \centering
	\subfigure[\textit{Nico} (VV1)]{\includegraphics[height=0.3\textwidth]{Figure_Jrn/Nico.png}}
    \quad
    \subfigure[\textit{Sir Frederic} (VV2)]{\includegraphics[height=0.3\textwidth]{Figure_Jrn/Frederick.png}}
    \caption{Volumetric Human Body sequences \cite{volograms2021} used in the AR experiment presented in \cite{zerman2021user}}
    \vspace{-1.5em}
    \label{Fig_HumanBodyDataset2}
\end{figure}

\begin{figure*}[ht]
	\centering
    \hspace{-2em}
	\subfigure[\textbf{VV1} - Mean Overlap Ratio in Relevant Cluster.]{
	\includegraphics[width=0.34\textwidth]{Figure_Jrn/PC_Nico_overlapRatio.png}}
	\quad
    \hspace{-2em}
	\subfigure[\textbf{VV1} - Mean Relevant Users.]{
		\includegraphics[width=0.34\textwidth]{Figure_Jrn/PC_Nico_relevantUsers.png}}
	\quad
    \hspace{-2em}
	\subfigure[\textbf{VV1} - Precision.]{
		\includegraphics[width=0.34\textwidth]{Figure_Jrn/PC_Nico_precision.png}}
		\quad
    \hspace{-2em}
    \\
    \hspace{-2em}
    \subfigure[\textbf{VV2} - Mean Overlap Ratio in Relevant Cluster.]{
	\includegraphics[width=0.34\textwidth]{Figure_Jrn/PC_Fredrick_overlapRatio.png}}
	\quad
    \hspace{-2em}
	\subfigure[\textbf{VV2} - Mean Relevant Users.]{
		\includegraphics[width=0.34\textwidth]{Figure_Jrn/PC_Fredrick_relevantUsers.png}}
	\quad
    \hspace{-2em}
	\subfigure[\textbf{VV2} - Precision.]{
		\includegraphics[width=0.34\textwidth]{Figure_Jrn/PC_Fredrick_precision.png}}
		\quad
    \hspace{-2em}
	\caption{Spherical clustering over time (chunk = 1 sec.) results per sequence VV1 (\textit{Nico}) and VV2 (\textit{Sir Fredrick}): performance comparison between ground-truth, and a subset of proposed metrics ($w_1$, $w_5$, $w_7$ and $w_8$).}
	\label{Fig_Vsense_1}
	\vspace{-1em}
\end{figure*}

Similarly to our previous investigations, we now apply to this new scenario the spherical clustering based on the subset of best-performing feature metrics, such as $w_1$. $w_5$, $w_7$ and $w_8$. We evaluate clusters in chunks of length 1$s$ with a time  similarity threshold of 0.8$s$ and the threshold values $G_{th}$ reported in Table~\ref{table_metrics}. At  each  chunk,  we  compute the average overlap ratio per relevant cluster (\ie cluster with at least two elements), the average of the relevant population and the precision of the detected clusters. Fig.~\ref{Fig_Vsense_1} shows these results as a function of time per each selected similarity metric, in particular, the first row refers to \textit{Nico} (VV1) while the second one to \textit{Sir Frederic} (VV2). Since viewers were allowed to drop the AR experience at any desired time, in the following we consider only the time window in which 75\% of the user population (15 out of 20 viewers) are still in the experiment: 63 and 83 seconds, respectively for VV1 and VV2. We observe that both the sequences have an initial moment of adjustment where viewers are displaying different portions of the content. This is detected by clusters based on the overlap ratio (\ie red line) which do not have a consistent pairwise overlap. For instance, Fig.~\ref{Fig_Vsense_1}~(a) shows in the first 40$s$ of the immersive experience for VV1 the average of overlap ratio within the main detected clusters has up and down for all the metrics, included the ground-truth. However, this behaviour stabilises around 40$s$ when the overlap ratio for the ground-truth metric converge to 1. Similarly, the performance metric detected by $w_1$ and $w_8$ reaches values above 0.6 with a very low variance for both the metrics. On the contrary, the overlap ratio of cluster detected by $w_5$ and $w_7$ has values below 0.5 and a more consistent variance over time. Indeed, these metrics in terms of relevant users (Fig.~\ref{Fig_Vsense_1}~(b)) generate bigger clusters compared to the ground-truth metric. In particular, $w_5$ considers almost the entire population at any given time in a big cluster, which is quite the opposite behaviour to the ground-truth metric. This metric indeed generates small relevant clusters most of the time; clusters based on $w_1$ and $w_8$ follow a very similar trend. These two metrics are also the best performing in terms of precision, as shown in Fig.~\ref{Fig_Vsense_1}~(c) with values always above 0.4.  A similar general behaviour is also observable for VV2 in the second line of Fig.~\ref{Fig_Vsense_1}. In this volumetric content, users explore more randomly during the first minute of the experience to end up having similar behaviour, in fact, clusters have a consistent overlap ratio (Fig.~\ref{Fig_Vsense_1}~(d)). As in the previous example, similarity metrics $w_1$ and $w_8$ are more precise in reflecting the ground-truth behaviour and thus, detecting viewers with similar behaviour and putting them within the same clusters. Finally, it is worth noticing that between 40 and 60 seconds, all the similarity metrics reach a higher overlap ratio compared to the ground-truth performance, in particular, metrics $w_1$ and $w_8$. This opens new questions to be further investigated as discussed in the following section.



==> _Sec_8_Discussion.tex <==
\section{Discussion and Future Work}
\label{sec_discussion}
We presented the main challenges of user behavioural analysis in a \sdof system due to the new settings and the added locomotion functionalities. However, behavioural analysis of \sdof users is not considered in the literature yet; as such, there is no reference metric available to detect viewers who are displaying the same portion of the content. Thus, we had to define a general ground-truth user similarity metric, such as \textit{overlap ratio}. To be as general as possible, we established the overlap as the percent of points displayed in common by two users. 
% This allowed us to apply the overlap ratio not only to volumetric content stored as point cloud but also as mesh \noteSR{not sure on this point}. 
This is fairly straightforward, albeit time-consuming, to compute for point cloud contents, in which each point is rendered separately. For other types of volumetric contents, determining the overlap ratio is not as simple. Considering the number of vertexes that fall into a given frustum could lead to misleading results when large faces between sparsely distributed vertexes are present.
Moreover, the
% The main drawback of this 
metric requires to render each volumetric video at any given time and for each viewer,  making its computation not trivial and intensely time-consuming. To overcome this issue and to assess users similarity in a simple and objective way, we investigate several similarity metrics considering different distance features and measurements. In detail, we investigate different features or combinations of them which consider users location in the virtual space and their viewing direction. First, we validate and test our similarity metrics via a clique-based clustering tool proposed for \tdof scenario on real navigation trajectory collected in a \sdof VR environment. Our extensive analysis shows that metrics based on multi-features better model and thus, detect similarity among users, reaching encouraging values of both overlap ratio and precision. 
Therefore, we tested their performance on a different kind of \sdof navigation trajectories. In this second dataset, viewers displayed volumetric content in an AR scenario through smartphones. Therefore, even if users were enabled with the same \sdof locomotion settings, the viewing device and the FoV were different. Despite these differences, our proposed similarity metrics are still good at identifying viewers who are displaying similar content. In this context not only a multi-feature metric is outperforming the others, but also the simplest one which is based only on the users location in the virtual space. This opens the gate to further investigations aimed at detecting user behavioural differences in a \sdof experience done in VR and AR settings. These are indeed essential to be exploited in efficient user-centric solutions for both immersive systems. Finally, it is worth mentioning that our ground-truth metric of similarity is very tight in detecting similar users, especially in an AR scenario. %\noteSR{Not so convinced to mention Fig. 7 here. Maybe is it better to move in the section before?}\lt{I think it fits well as it leads to the open challenges} 
%As an example, Fig.~\ref{Fig_Vsense_2} shows the number of single clusters detected over time by the overlap ratio (\ie red line) and the sub-set of most performing similarity metrics for both the volumetric sequences of the second analysed dataset. In particular, in VV2 (Fig.~\ref{Fig_Vsense_2}~(b)), the clique-based clustering based on the overlap ratio does not detect similar users such that the majority of the population are put in a single cluster. Therefore, further analysis is needed to test if in this scenario a different overlap threshold better model similarity among users. 

==> _Sec_8_ablation_study.tex <==
\section{Ablation Study}
\label{sec_ablationStudy}
As part of our validation problem, we also present an ablation study to tune the best set of parameters per each similarity metric. Equipped with the threshold values per each similarity metrics given in Table~\ref{table_metrics}, we run a frame-based clustering to select the best set or sub-set of regulators $\alpha$, $\beta$ and $\sigma$. We test their performance in the following range of values $[0, 0.05, 0.1, 0.125, 0.2, 0.25, 0.5, 1, 2]$, based on navigation trajectories collected for reference content of the dataset describe in Section~\ref{sec_dataset}. We used the performance metrics described in Section~\ref{sec_performance} such as overlap ratio, precision and relevant population. In detail, we average the final performance of clusters obtained by all similarity metrics over time and across content.\\
\textbf{Single-feature metrics}\\
For single-feature metrics ($w_1-w_4$), we notice a very small variance in term of performance per each similarity metrics. Therefore, we decided to select $\alpha = 1$ for this set of metrics. \\
%In particular, we collected in Table~\ref{table_single_metrics} the performance given by each similarity metric in our analysis. We can notice that $w_1$ outperform in terms of overlap ratio $O$ and precision even if they are quite low (0.65 and 0.44, respectively). On the contrary, $w_2$ reaches the best results in terms of relevant clustered population \textcolor{red}{and \ac{GDI}}.\\
\textbf{Multi-feature metrics}\\
More challenging is instead the selection parameters for multi-feature metrics ($w_5-w_8$). Each similarity metric depends indeed on three parameters: $\alpha$, $\beta$ and $\gamma$. We first select three sets of parameters taking into account only navigation trajectories for reference content: one group of parameters (\textcolor{set1}{set 1}) based on the maximum overlap ratio, the second (\textcolor{set2}{set 2}) depending on the relevant clustered population and finally, the last group (\textcolor{set3}{set 3}) as the one set of parameters reaching the highest precision. As example, we report in Fig.~\ref{Fig_parameter_selection_w8} the selection of these three sets of parameters for the similarity metric $w_7$. Then, we test these values on all the available trajectories included in the analysed dataset to finally select the best set of parameters. Table~\ref{table_metrics_multi_feature} provide all the performance of the multi-feature similarity metrics obtained by the three selected sets of parameters. Since there is no a particular configuration that outperform in terms of overlap ratio, relevant population and precision, we decided to select all regulators selected in \textcolor{set3}{set 3}. This configuration indeed ensure a good balance of overlap ratio and relevant population for all the similarity metrics and ensure the highest value of precision. 
\begin{figure*}[th]
	\centering
	\hspace{-1em}
	\subfigure[Overlap Ratio]{
	\includegraphics[width=0.32\textwidth]{Figure_Jrn/Parameter_sel_ov_w7_new.png}}
	\quad
    \hspace{-1em}
	\subfigure[Relevant population]{
		\includegraphics[width=0.32\textwidth]{Figure_Jrn/Parameter_sel_user_w7_new.png}}
	\quad
    \hspace{-1em}
	\subfigure[Precision]{ 
		\includegraphics[width=0.32\textwidth]{Figure_Jrn/Parameter_sel_P_w7_new.png}}
	\caption{Example of parameter selection for $w_7$ with $\beta = 0.5$. Values \textcolor{set1}{set 1} selected based on max overlap, \textcolor{set2}{set 2} max clustered users, \textcolor{set3}{set 3} based on precision.}
	\label{Fig_parameter_selection_w8}
\end{figure*}
%\begin{figure*}[h]
%	\centering
%	\hspace{-1em}
%	\subfigure[Mean Overlap Ratio per cluster]{
%	\includegraphics[width=0.32\textwidth]{Figure_Jrn/Boxplot_overlap_Parameter.png}}
%	\quad
%    \hspace{-1em}
%	\subfigure[Relevant clustered population]{
%		\includegraphics[width=0.32\textwidth]{Figure_Jrn/Boxplot_users_Parameter.png}}
%	\quad
%    \hspace{-1em}
%	\subfigure[Precision]{ 
%		\includegraphics[width=0.315\textwidth]{Figure_Jrn/Boxplot_precision_Parameter.png}}
%	\caption{Performance frame-based clustering parameter selection. \noteSR{To be fixed} \noteSR{Do we want to have only a  table instead of these figures so I can also put all the values of $\alpha$, $\beta$ and $\gamma$?}}
%	\label{fig_boxplot}
%\end{figure*}

\input{table_parameters}

